Is there an order-barrier $p\leq2$ for time integration in computational elasto-plasticity?

This paper is devoted to the question, whether there is an order barrier $p\leq2$ for time integration in computational elasto-plasticity. In the analysis we use an implicit Runge-Kutta (RK) method of order $p=3$ for integrating the evolution equations of plastic flow within a nonlinear finite element framework. We show that two novel algorithmic conditions are necessary to overcome the order barrier, (i) total strains must have the same order in time as the time integrator itself, (ii) accurate initial data must be calculated via detecting the elastic-plastic switching point (SP) in the predictor step. Condition (i) is for a \emph{consistent} coupling of the global boundary value problem (BVP) with the local initial value problems (IVP) via displacements/strains. Condition (ii) generates consistent initial data of the IVPs. The third condition, which is not algorithmic but physical in nature, is that (iii) the total strain path in time must be smooth such that condition (i) can be fulfilled at all. This requirement is met by materials showing a sufficiently smooth elastic-plastic transition in the stress-strain curve. We propose effective means to fulfil conditions (i) and (ii). We show in finite element simulations that, if condition (iii) is additionally met, the present method yields the full, theoretical convergence order 3 thus overcoming the barrier $p\leq 2$ for the first time. The observed speed-up for a 3rd order RK method is considerable compared with Backward Euler.

==> SimpleShearExample.tex <==
%----------------------------------------------------------------------------
\subsection{Simple shear}
\label{ElPl-Shear}
%----------------------------------------------------------------------------

The first example is the elasto-plastic simple shear deformation of a cube discretized by one
hexahedron element of side length $L$ as displayed in Fig. \ref{fig:SimpleShear}.
The boundary conditions for shear in the $Y$-$Z$-plane are chosen to avoid
rigid body motions and to ensure a homogeneous deformation state.
The nodes at $z=L$ are subject to displacement control in $y$-direction by $u_y(t) = 0.001[L]\, t$\footnote{Since the plasticity model is 
rate-independent, the deformation history is parameterized by a dimensionless time.}. Material parameters for von-Mises elasto-plasticity 
with linear isotropic hardening are listed in Tab. \ref{tab:MatShearliniso}. The convergence analysis is based on stresses at times $t=\{20,60,100\}$,
the results are displayed in Tab.~\ref{tab:KonvergenzShearliniso} and in Fig.~\ref{fig:KonvergenzShearliniso}.

% The switching point in this test is at $t_{\mbox{\scriptsize SP}}=6.5763$.
% Reference solutions for error and convergence analysis are listed in
% Tab. \ref{tab:Shearlinisoexakt} obtained by RIIa-q-SP along with a time step size $\Delta t = 0.05$.\\
%

\begin{Figure}[htbp]
   \begin{minipage}{15.0cm}
   \centering
      \scalebox{.35}{\input{2nd.pstex_t}}
   \end{minipage}
\caption{Simple shear: undeformed and deformed state.\label{fig:SimpleShear}}
\end{Figure}

\begin{Table}[htbp]
\center
\renewcommand{\arraystretch}{1.4}
%\begin{tabular}{llcc}
\begin{tabular}{cccccc}
\hline
 $E$ $({\text{N}}/{\text{mm}^2})$                            &
 $\nu$ $(1)$                                                 &
 $\sigma_Y$ $({\text{N}}/{\text{mm}^2})$                     &
 $\sigma_\infty - \sigma_Y$ $({\text{N}}/{\text{mm}^2})$     &
 $H$ $({\text{N}}/{\text{mm}^2})$                            &
 $\delta$  $(1)$                                            \\
\hline
$210\,000$   &   $0.3$   &   $460$   &   $0$    &   $10000$   &  $0$\\
 \hline
\end{tabular}
\caption{Simple shear: elasto-plastic material parameters.}\label{tab:MatShearliniso}
\end{Table}

%Da die Radau IIA-Verfahren mit quadratischer Interpolation die Referenzl\ösung schon mit gr\ö sseren Schrittweiten erreichen,
\begin{Table}[htbp]
\renewcommand{\arraystretch}{1.4}
\center
%\begin{tabular}{c|ccccccc}
\begin{tabular}{rccccccccc}
   \hline
           time $t$ \,\,      & \hspace*{1mm} & BE    & \hspace*{2mm}  & RIIa-l  & RIIa-l-SP  & \hspace*{2mm} &  RIIa-q & \cellcolor{hellgrau} RIIa-q-SP  & \cellcolor{hellgrau} RIIa-q-exSP \\
   \hline $\phantom{1}20$\, : &               & 0.91  &                & 1.95    & 1.97       &               &  2.31   & \cellcolor{hellgrau} 3.04 & \cellcolor{hellgrau} 3.25 \\
          $\phantom{1}60$\, : &               & 0.99  &                & 1.95    & 1.95       &               &  2.42   & \cellcolor{hellgrau} 3.10 & \cellcolor{hellgrau} 3.14 \\
                    $100$\, : &               & 1.00  &                & 1.95    & 1.95       &               &  2.32   & \cellcolor{hellgrau} 3.14 & \cellcolor{hellgrau} 3.17 \\
 \hline
\end{tabular}
\caption{Simple shear: mean convergence order of $e(\bS)$ for different integration schemes.\label{tab:KonvergenzShearliniso}}
\end{Table}

\begin{Figure}[htbp]
  \begin{minipage}{15.5cm}
  {\centering
   \includegraphics[width=.45\textwidth, angle=0, clip=]{Shear_liniso_sig_t020} \hspace*{4mm}
%   \includegraphics[width=7.5cm, angle=0, clip=]{Shear_liniso_sig_t060-bb}\\
   \includegraphics[width=.45\textwidth, angle=0, clip=]{Shear_liniso_sig_t100}
   \\
  }
  \end{minipage}
  \caption{Simple shear. Error $e(\bS)$ versus time step-size $\Delta t$ at time $t=20$ (left) and at $t=100$ (right).
  \label{fig:KonvergenzShearliniso}}
\end{Figure}

Backward Euler shows linear convergence, Radau IIa using linear interpolation results in order reduction 
to order 2, which cannot be cured by switching point detection. More accurate results are achieved for 
quadratic interpolation, but the convergence is not strictly uniform in that case. 
For quadratic interpolation combined with switching point detection, the full convergence order 3 is obtained. 
There is not a big difference between switching point detection based on extrapolation of strain compared with 
RIIa-q-SP. 
\\[2mm]
A comparison of errors at different times $t=\{20, 100\}$ in Fig.~\ref{fig:KonvergenzShearliniso} shows, that 
the error accumulates in plastic deformation history, such that higher order methods become increasingly attractive 
at later times. At $t=100$ for example, third order Radau IIa is already more accurate for time step size $\Delta t=20$ 
than Backward-Euler for $\Delta t=0.125$ and is of the same accuracy as Radau IIa for $\Delta t=1.05$ suffering from 
order reduction.

==> command.tex <==
\newcommand\leerseite{\newpage\thispagestyle{empty}\hspace{1cm}\newpage}
\renewcommand{\labelitemi}{$\bullet$}
\newcommand {\fat}[1]{{\mbox{\boldmath{$#1$}}}}
\newcommand {\fa}[1]{{\mathbf{#1}}}
\newcommand {\dx}{\text{d}\mathbf{x}}
\newcommand {\dX}{\text{d}\mathbf{X}}
\newcommand {\dv}{\text{d}v}
\newcommand {\da}{\text{d}\mathbf{a}}
\newcommand {\df}[1]{\text{d}\mathbf{#1}}
\newcommand {\dn}[1]{\text{d}#1}
\newcommand{\I}{\int\limits}
\newcommand{\Sum}{\sum\limits}
\newcommand{\Prod}{\prod\limits}
\newcommand{\sig}{{\mbox{\boldmath{$\sigma$}}}}
\newcommand{\sigd}{{\mbox{\boldmath{$\sigma^D$}}}}
\newcommand{\eps}{\fat{\varepsilon}}
\newcommand{\vep}[1]{\fat{\varepsilon}_{#1}}
%\newcommand{\ev}{\text{e}_{\text{v}}}
\newcommand{\evn}{\text{e}_{\text{v}n}}
\newcommand{\dev}{\dot{\text{e}}_{\text{v}}}
\newcommand{\fS}{\mathbf{S}}
\newcommand{\qf}{q_1q_2{f^{\ast}}}
\newcommand{\argu}{\biggl(\frac{q_2\,\JH{1}}{2\,\yev}\biggl)}
\newcommand{\trace}{\text{tr}(\sig)}
\newcommand {\parziell}[2]{\frac{\partial#1}{\partial#2}}
\newcommand {\dparziell}[2]{\dfrac{\partial#1}{\partial#2}}
\newcommand {\parzer}[3]{\frac{\partial^2#1}{\partial#2\;\partial#3}}
\newcommand {\parzerer}[2]{\frac{\partial^2#1}{\partial#2^2}}
\newcommand{\lam}{\Delta\lambda}
\newcommand{\ter}[1]{$#1^\text{ter}$}
\renewcommand{\det}[1]{\text{det}(#1)}
\newcommand{\assembly}{\overset{\text{\tiny $nelem$}}{\underset{\text{\tiny
$e=1$}}{\text{{\LARGE $\fa{A}$}}}}}
\newcommand{\JD}[1]{J_#1{\mbox{\small$[\sigd]$}}}
\newcommand{\JH}[1]{J_#1{\mbox{\small$[\sig]$}}}
\newcommand{\yev}{y{ \mbox{\small $[\ev]$}}}
\newcommand{\J}[2]{J_#1{\mbox{\small$[#2]$}}}
\newcommand{\expr}{\biggl(\frac{q_2\,\JH{1}}{2\,y}\biggl)}%\text{tr}(\sig)}
\newcommand{\Aev}{A\mbox{\small$[\ev]$}}
%eigene
\newcommand{\sigeq}{\sig^\text{eq}}
\newcommand{\sigov}{\sig^\text{ov}}
%Umlaute
%\newcommand{\ö}{\"{o}}
%\newcommand{\ä}{\"{a}}
%\newcommand{\ü}{\"{u}}
%\newcommand{\Ö}{\"{O}}
%\newcommand{\Ä}{\"{A}}
%\newcommand{\Ü}{\"{U}}
%doppelt
\newcommand{\Id}{\mathbb{I}\text{d}}
\newcommand{\Is}{\mathbb{I}\text{s}}
\newcommand{\1}{\mathbf{1}}
\newcommand{\C}{\mathbb{C}}
\newcommand{\Cep}{\mathbb{C}_{n+1}^{ep}}
\newcommand{\Ck}{\mathbb{C}_{n+1}^{ep,k}}
\newcommand{\Amat}{\mathbb{A}}
\newcommand{\Bmat}{\mathbb{B}}
\newcommand{\devP}{\mathbb{P}}
\newcommand{\Real}{\mathbb{R}}
%K
\newcommand{\dK}{\hat{K'}}
\newcommand{\ddK}{\hat{K''}}
%e
\newcommand{\ee}{\mathbf{e}}
\newcommand{\ev}{\mathbf{e}^\text{v}}
\newcommand{\dtev}{\dot{\mathbf{e}}^\text{v}}
\newcommand{\enp}{\mathbf{e}_{n+1}}  %e_n+1
%\newcommand{\en}{\mathbf{e}_n}       %e_n
%ep
%\newcommand{\ep}{\mathbf{e}^p}
\newcommand{\epnp}{\mathbf{e}^{p}_{n+1}} %e^p_n+1
\newcommand{\epm}{\mathbf{e}^{p}_{n-1}}
\newcommand{\epnptr}{\mathbf{e}^{p,tr}_{n+1}} %e^p_n+1^tr
%\newcommand{\epnh}{\mathbf{e}^{p}_{n+\frac{1}{2}}}
\newcommand{\epnh}{\mathbf{e}^{p}_{n+\text{\tiny{1/2}}}}
\newcommand{\epn}{\mathbf{e}^{p}_n} %e^p_n
\newcommand{\Ep}{\mathbf{E}^p}
\newcommand{\Ev}{\mathbf{E}^\text{v}}
%alpha
\newcommand{\anp}{\alpha_{n+1}}
\newcommand{\am}{\alpha_{n-1}}
\newcommand{\anptr}{\alpha_{n+1}^{tr}}
\newcommand{\alhtr}{\alpha_{n+\text{\tiny{1/2}}}^{tr}}
\newcommand{\alh}{\alpha_{n+\text{\tiny{1/2}}}}
%s
\newcommand{\sn}{\mathbf{s}_n}
\newcommand{\snp}{\mathbf{s}_{n+1}} %s_n+1
%\newcommand{\snh}{\mathbf{s}_{n+\frac{1}{2}}}
\newcommand{\snh}{\mathbf{s}_{n+\text{\tiny{1/2}}}}
\newcommand{\snhtr}{\mathbf{s}_{n+\text{\tiny{1/2}}}^{tr}}
\newcommand{\s}{\mathbf{s}}
\newcommand{\snptr}{\mathbf{s}_{n+1}^{tr}}
\newcommand{\snpf}{\mathbf{s}_{n+1}^{tr,1}}
%\newcommand{\snhtr}{\mathbf{s}_{n+\frac{1}{2}}^{tr}}
%\newcommand{\snhtr}{\mathbf{s}_{n+\text{\tiny{1/2}}}}
%eps
\newcommand{\epse}{\fat{\varepsilon}_\text{e}}
\newcommand{\epsv}{\fat{\varepsilon}_\text{v}}
\newcommand{\epsen}{\fat{\varepsilon}^{e}_n}
\newcommand{\epsenp}{\fat{\varepsilon}^e_{n+1}}
\newcommand{\epsp}{\fat{\varepsilon}^{e}}
\newcommand{\epsnp}{\fat{\varepsilon}_{n+1}}
%n
\newcommand{\n}{\mathbf{n}_{n+1}}
%\newcommand{\nh}{\mathbf{n}_{n+\frac{1}{2}}}
\newcommand{\nh}{\mathbf{n}_{n+\text{\tiny{1/2}}}}
\newcommand{\N}{\mathbf{N}}
%delta
\newcommand{\du}{{\Delta u}}
\newcommand{\dz}{{\Delta z}}
\newcommand{\ddz}{{\Delta^2 z}}
%phi
\newcommand{\phihtr}{\phi_{n+\text{\tiny{1/2}}}^{tr}}
%andere
\newcommand{\be}{\fat{\beta}}
\newcommand{\Edom}{\mathcal{E}}
\newcommand{\alphah}{\alpha_{n+\text{\tiny{1/2}}}}
\newcommand{\alphan}{\alpha_{n+1}}
\newcommand{\x}{\mathbf{x}}
\newcommand{\kO}{\mathcal{O}}
\newcommand{\hateq}{\,\,\hat{=}\,\,}
%text
\newcommand{\tr}{\text{tr}}
\newcommand{\deviat}{\text{dev}}



==> ftemplate_js_2.tex <==

%========================================================================
%          ***  First Page of Paper  ***
%========================================================================
\thispagestyle{empty}

\ce{{\Large UNIVERSITY OF DUISBURG-ESSEN}
\phantom{x}
{\large CAMPUS ESSEN}}

\begin{figure}[htb]
\unitlength1cm
\begin{picture}(14,5)
\put(6.4,1.50){\scalebox{0.48}{\includegraphics{penrose_bw.eps}}}
\put(10,4){Universit\"at Duisburg-Essen}
\put(10,3.5){Institut f\"ur Mechanik}
\put(10,3){Fakult\"at f\"ur Ingenieurwissenschaften}
\put(10,2.5){Abteilung Bauwissenschaften}
\put(10,1.5){Prof. Dr.-Ing. habil. J. Schr\"oder}
\end{picture}
\end{figure}

\vspace*{2cm}
\begin{center}
{\Huge
Paper Template for the Reports of the Institute for Mechanics.
} 

{\bf \large
\medskip
Subtitle of the report.
}

\vspace{1.0cm}

{\large By J\"org Schr\"oder}


\vspace{6.0cm}

\renewcommand{\arraystretch}{1.5}
\begin{tabular}{|c|c|}
\hline
{\bf Report -- Preprint} & {\bf No. XX (2010)} \\
\hline
\end{tabular}

\vspace{.50cm}
Editor: Prof. Dr.-Ing. J\"org Schr\"oder
\vspace{2.0cm}

{\large Universit\"atsstra\ss e 15, 45117 Essen, Germany}

\end{center}

\newpage

